Compressed Error HARQ: Feedback Communication on Noise-Asymmetric Channels

In modern communication systems with feedback, there are increasingly more scenarios where the transmitter has much less power than the receiver (e.g., medical implant devices), which we refer to as noise-asymmetric channels. For such channels, the feedback link is of higher quality than the forward link. However, feedback schemes for cellular communications, such as hybrid ARQ, do not fully utilize the high-quality feedback link. To this end, we introduce Compressed Error Hybrid ARQ, a generalization of hybrid ARQ tailored for noise-asymmetric channels; the receiver sends its estimated message to the transmitter, and the transmitter harmoniously switches between hybrid ARQ and compressed error retransmission. We show that our proposed method significantly improves reliability, latency, and spectral efficiency compared to the conventional hybrid ARQ in various practical scenarios where the transmitter is resource-constrained.

==> fharq_framework.tex <==
% TODO: add some total flow for introducing the F-HARQ framework. Can be a material bank for future writing. 



\subsection{Design Goal}
Our major design goal, is to optimize throughput and latency, under asymmetric channel conditions, for real communication ports such as cellular, Wifi and bluetooth. 


% Why optimize throughput and latency
most communication systems optimize for spectrum efficiency. However, spectrum efriciency can be very 



Number of round is critical for 

% why specific communication layers.




\subsection{System Description and Objective}





\subsection{Literature Comparison Study}





\subsection{Motivations}




\subsection{Algorithm Design}




\subsection{Contributions}









==> practical_considerations.tex <==
\section{Practical considerations}\label{sec:practical}

In this section, we examine some of the prevalent challenges encountered in the practical implementation of existing feedback codes and explain how CE-HARQ addresses these bottlenecks.

% (I) AIC - variable length vs. Ours - fixed length at every transmission. (II) Spectral efficiency - their metric - is not a practical metric. # of rounds. 

\subsection{Adaptive and Iterative compression}
% (I) Need to think about Message or Error , (II) Sol: Threshold - sparsity level. 



% The retransmissions in a HARQ scheme can be viewed as an extra layer of repetition coding which improves the decoding probability by increasing the effective SNR. In contrast, schemes like AIC iteratively transmit the compressed error vector every round, reducing the number of channel uses. The error compression does not have an effect on legacy retransmission schemes such as ARQ, where there is no SNR gain with retransmission. But modern retransmission frameworks such as HARQ suffer a noticeable loss in SNR gain by choosing error compression instead of HARQ, especially when the maximum number of retransmissions allowed is small. The error compression enables CE-HARQ to obtain coding gains by using a lower rate FEC code. However, it is not straightforward whether this coding gain overcomes the loss of SNR gain. Hence, the proposed selection mechanism for CE-HARQ based on the sparsity of the error vector $|e^{(i)}|$ addresses this trade-off to choose optimal retransmission scheme for each round.
% \looseness=-1


The retransmissions in a HARQ scheme can be viewed as an extra layer of repetition coding which improves the decoding probability by increasing the effective SNR. In contrast, transmitting the compressed error vector enables CE-HARQ to obtain coding gain by allowing the use of a lower rate FEC code, obtaining coding gain. As demonstrated in Figure \ref{fig:toy_example}, switching to the compressed error scheme is beneficial only when the error vector is sufficiently sparse, and the achieved coding gain is greater than the SNR gain offered by HARQ. Towards this, we propose an adaptive selection mechanism that chooses the optimal retransmission scheme based on the sparsity of the error vector $|e^{(i)}|$.

The optimal sparsity level $\tau^\star$ varies dynamically with the SNR and number of remaining rounds: if $|e^{(i)}| > \tau^\star$, it is better to continue with HARQ. Once the required sparsity is observed, it is advantageous to leverage the coding gain obtained by transmitting the compressed error using a low-rate FEC code. Analytically determining the optimal threshold $\tau^\star$ is a challenging task. In short block length regime, the optimality of both source and channel coding techniques do not hold true, which impedes the analytic estimation of the error rate for a given rate and SNR. However, it is straightforward to compute using Monte Carlo simulations. We discuss the details of both approaches in detail in Appendix A.

% Entropy coding -> might lead to larger # of errors. Previous error. 
\subsection{Fallback mechanism through error monitoring}
One significant drawback of using source coding techniques such as AC to compress the error vector is the large number of errors encountered in the decompressed vector when an error occurs in the compressed vector. This is known as the avalanche effect \cite{feistel1973cryptography} and is a desirable property in cryptography. But this is highly detrimental for compressed error based feedback schemes such as CEC and AIC. Due to this effect, it cannot be guaranteed that the number of errors in round $i+1$ is less than that in round $i$. To mitigate this issue, CE-HARQ employs a fallback mechanism by continually monitoring the error. 

By continuously monitoring the sparsity of error vector, the transmitter decides whether the previous retransmission improved or degraded the estimate. If the estimate is degraded, instead of compressing $e^{(i+1)}$, the transmitter falls back to HARQ and retransmits $e^{(i)}$ to improve the estimate at the receiver. This fallback mechanism ensures that the number of errors in the estimate decreases continuously over retransmissions, which is crucial for practical systems, and the iterative compression is done only when the new estimate is better than the previous estimate.

% Consider round $i$, where the transmitter compresses and sends the error vector $e^{(i)}$ to the receiver. The receiver then estimates the error as $\hat{e}^{(i)}$ and computes the corrected vector as $\hat{u}^{(i+1)} = \hat{u}^{(i)} + \hat{e}^{(i)}$. After receiving the feedback of the $i^{th}$ round $\hat{m}^{i+1}$, the transmitter computes the error $e^{(i+1)} = u \oplus \hat{u}^{i+1}$. By comparing the errors $e^{(i+1)}$ and $e^{(i)}$, the transmitter decides whether the previous retransmission improved or degraded the estimate. If the estimate is degraded, instead of compressing $e^{(i+1)}$, the transmitter falls back to HARQ and retransmits $e^{(i)}$ to improve the estimate at the receiver. This fallback mechanism ensures that the number of errors in the estimate decreases continuously over retransmissions, which is crucial for practical systems, and the iterative compression is done only when the new estimate is better than the previous estimate. Based on our experiments, it is observed that such fallback mechanism is essential for ensuring reliable performance when the total number of retransmissions is low.

% source-coding & channel-coding: we fix the channel coding rate. Entropy coding -> conv -> channel coding. 
% \subsection{PHY/MAC separation}
% The ability to separate changes in the retransmission scheme between the PHY and MAC layers is a desirable property in many real-world systems. The CEC \cite{ooi1998fast} and AIC \cite{perotti2021accumulative} schemes are agnostic to such constraints. In contrast, CE-HARQ scheme is suitable for both PHY and MAC changes, as well as can limit all changes to only MAC layer. In systems with fixed PHY layer, CE-HARQ encodes the compressed error length $K$, protecting the compressed error with rate $\sfrac{H(e^{(i)})}{K}$. But when PHY modifications are allowed, CE-HARQ encodes directly to length $N$, providing superior protection with rate $\sfrac{H(e^{(i)})}{N}$, as demonstrated in Fig. ?? in Appendix ??.

% In a retransmission scheme, the transmitter must choose the message for next round based on the feedback received. In AIC, the error vector is compressed to entropy after each round regardless of the feedback. While this is beneficial for improving spectral efficiency, in practice, the SNR gain achieved by using HARQ is lost because of the continual compression. In CE-HARQ, the compression achieved directly affects the FEC coding gain. Hence it is important to consider this trade-off between SNR gain and the FEC coding gain while selecting the retransmission scheme. If the error vector is not sufficiently sparse, it may not be possible to achieve the necessary compression level for good coding gain, resulting in performance inferior to  HARQ. Therefore, after each round, the sparsity of the error vector is compared to a threshold $\tau$ that dynamically varies with SNR and the number of rounds remaining. 

% In a retransmission scheme, the transmitter must choose the message for next round based on the feedback received. In AIC, the error vector is compressed to entropy after each round regardless of the feedback. While this is beneficial for improving spectral efficiency, in practice, the SNR gain achieved by using HARQ is lost because of the continual compression. In CE-HARQ, the compression achieved directly affects the FEC coding gain. Hence it is important to consider this trade-off between SNR gain and the FEC coding gain while selecting the retransmission scheme. If the error vector is not sufficiently sparse, it may not be possible to achieve the necessary compression level for good coding gain, resulting in performance inferior to  HARQ. Therefore, after each round, the sparsity of the error vector is compared to a threshold $\tau$ that dynamically varies with SNR and the number of rounds remaining. 

% Determining the optimal threshold $\tau$ dynamically is a challenging task due to the various factors involved. At very short block lengths, the optimality of both source and channel coding techniques do not hold true, and therefore,
% estimating the error rate for a given rate and SNR analytically not possible. However, the method for choosing the threshold $\tau$ based on asymptotic behavior can be easily extended to short block length cases using Monte Carlo simulation data.


